MARVEL: Unlocking the Multi-Modal Capability of Dense Retrieval via Visual Module Plugin

This paper proposes Multi-modAl Retrieval model via Visual modulE pLugin (MARVEL), which learns an embedding space for queries and multi-modal documents to conduct retrieval. MARVEL encodes queries and multi-modal documents with a unified encoder model, which helps to alleviate the modality gap between images and texts. Specifically, we enable the image understanding ability of the well-trained dense retriever, T5-ANCE, by incorporating the visual module's encoded image features as its inputs. To facilitate the multi-modal retrieval tasks, we build the ClueWeb22-MM dataset based on the ClueWeb22 dataset, which regards anchor texts as queries, and extracts the related text and image documents from anchor-linked web pages. Our experiments show that MARVEL significantly outperforms the state-of-the-art methods on the multi-modal retrieval dataset WebQA and ClueWeb22-MM. MARVEL provides an opportunity to broaden the advantages of text retrieval to the multi-modal scenario. Besides, we also illustrate that the language model has the ability to extract image semantics and partly map the image features to the input word embedding space. All codes are available at https://github.com/OpenMatch/MARVEL.

==> ethics_statement.tex <==
\section{Ethics Statement}
The paper does not raise any ethical considerations. It introduces ClueWeb22-MM as a resource to support the advancement of research in multi-modal retrieval within the academic community. This dataset is constructed from the ClueWeb22~\cite{overwijk2022clueweb22} dataset, for which appropriate licensing has been obtained. Additionally, this paper utilizes WebQA~\cite{chang2022webqa}, a widely used open-source dataset in multi-modal retrieval research. Consequently, the models trained on these datasets are not associated with foreseeable risks. Furthermore, to ensure the reproducibility of experiments, all source code will be made publicly available.


==> figure/embedding.tex <==
\begin{figure}
    \centering
    \subfigure[zero-shot-image.] { \label{fig:embed:zs-image} 
    \includegraphics[width=0.48\linewidth]{image/zero-shot_image.png}}
    \subfigure[zero-shot-text.] { \label{fig:embed:zs-text} 
    \includegraphics[width=0.48\linewidth]{image/zero-shot_text.png}}

    \subfigure[first-image.] { \label{fig:embed:f-image} 
    \includegraphics[width=0.48\linewidth]{image/first-image.png}}
    \subfigure[first-text.] { \label{fig:embed:f-text}
    \includegraphics[width=0.48\linewidth]{image/first-text.png}}

    \subfigure[second-image.] { \label{fig:embed:s-image} 
    \includegraphics[width=0.48\linewidth]{image/second-image.png}}
    \subfigure[second-text.] { \label{fig:embed:s-text}
    \includegraphics[width=0.48\linewidth]{image/second-text.png}}
    
    \caption{Embedding.}
    \label{fig:embed_tsne}
\end{figure}

==> figure/image_caption_attention.tex <==
\begin{figure}[t]
    \centering
    \subfigure[Attention Distribution of Image Features.] { \label{fig:attention:image} 
    \includegraphics[width=0.48\linewidth]
    {image/image_attention.png}}  
    \subfigure[Attention Distribution of Image Captions.] { \label{fig:attention:caption} 
    \includegraphics[width=0.48\linewidth]{image/caption_attention.png}}

    
    \caption{Image Feature and Image Caption Selection Effectiveness. Figure~\ref{fig:attention:image} shows the distribution of attention weights on image features, sorted by their weights; Figure~\ref{fig:attention:caption} shows the distribution of attention weights on image captions.}
    \label{fig:attention}
\end{figure}

==> figure/retrievalcase.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{image/webqa_retrieval_case.pdf}
\caption{Case Study on MARVEL Retrieval Effectiveness. We present one case each from WebQA and ClueWeb22-MM and show top-5 retrieved multi-modal documents from MARVEL and UniVL-DR. The ground-truth documents are emphasized.}
\label{fig:top5case}
\end{figure*}
